Endovascular Detection of Catheter-Thrombus Contact by Vacuum Excitation

Objective: The objective of this work is to introduce and demonstrate the effectiveness of a novel sensing modality for contact detection between an off-the-shelf aspiration catheter and a thrombus. Methods: A custom robotic actuator with a pressure sensor was used to generate an oscillatory vacuum excitation and sense the pressure inside the extracorporeal portion of the catheter. Vacuum pressure profiles and robotic motion data were used to train a support vector machine (SVM) classification model to detect contact between the aspiration catheter tip and a mock thrombus. Validation consisted of benchtop accuracy verification, as well as user study comparison to the current standard of angiographic presentation. Results: Benchtop accuracy of the sensing modality was shown to be 99.67%. The user study demonstrated statistically significant improvement in identifying catheter-thrombus contact compared to the current standard. The odds ratio of successful detection of clot contact was 2.86 (p=0.03) when using the proposed sensory method compared to without it. Conclusion: The results of this work indicate that the proposed sensing modality can offer intraoperative feedback to interventionalists that can improve their ability to detect contact between the distal tip of a catheter and a thrombus. Significance: By offering a relatively low-cost technology that affords off-the-shelf aspiration catheters as clot-detecting sensors, interventionalists can improve the first-pass effect of the mechanical thrombectomy procedure while reducing procedural times and mental burden.

==> PaperFmt/Tables_preamble.tex <==
%============= TABLES STUFF BELOW ======================
\usepackage{array}
\usepackage{booktabs}
\usepackage{floatrow}  %needed to push location of table caption above table https://tex.stackexchange.com/questions/22751/how-to-force-table-caption-on-top
\floatsetup[table]{capposition=top}
\usepackage{multirow}  %needed for multi-row table
\usepackage{tabularx}  %needed for tabularx environment for nicer column alignment in a table
\usepackage{colortbl} %needed for colored cells in Tabularx see http://tex.stackexchange.com/questions/148784/colored-diagonal-divided-table-cell
\usepackage{tabu}
\usepackage{footnote}% placed after tabularx so it does not conflict
\usepackage{arydshln} % this one is required for dashed line in table
%------------------------------------------------
% Define a new line thickness for tables see http://tex.stackexchange.com/questions/41758/how-can-i-reproduce-this-table-with-thick-lines
\makeatletter
\newcommand{\thickhline}{%
    \noalign {\ifnum 0=`}\fi \hrule height 2pt
    \futurelet \reserved@a \@xhline
}
\newcolumntype{"}{@{\hskip\tabcolsep\vrule width 2pt\hskip\tabcolsep}}
\makeatother

==> PaperFmt/lists_preamble.tex <==
\usepackage{enumerate}
%\usepackage{enumitem}
% equation with section numbering
%\numberwithin{equation}{section}
% Customized enumerate list spacing
\newenvironment{packed_enum}
{\begin{enumerate}[(a)]
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

\newenvironment{packed_enum_i}
{\begin{enumerate}[(i)]
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

%\newenvironment{packed_enum_arabic}
%{\begin{enumerate}[label=\arabic*.)]
%  \setlength{\itemsep}{1pt}
%  \setlength{\parskip}{0pt}
%  \setlength{\parsep}{0pt}
%}{\end{enumerate}}

\newenvironment{journal_packed_enum}
{\begin{enumerate}[label= J.\arabic*]
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

\newenvironment{conf_packed_enum}
{\begin{enumerate}[label= C.\arabic*]
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

\newenvironment{thesis_packed_enum}
{\begin{enumerate}[label= T.\arabic*]
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

\newenvironment{book_chapter_enum}
{\begin{enumerate}[label= BC.\arabic*]
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

\newenvironment{Abstract_enum}
{\begin{enumerate}[label= A.\arabic*]
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

\newenvironment{granted_patent_enum}
{\begin{enumerate}[label= GP.\arabic*]
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

\newenvironment{Licensed_enum}
{\begin{enumerate}[label= L.\arabic*]
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

\newenvironment{pending_patent_enum}
{\begin{enumerate}[label= P.\arabic*]
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

\newenvironment{packed_bullet}
{\begin{itemize}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{itemize}}

\newenvironment{packed_itemize}
{\begin{itemize}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{itemize}}


==> PaperFmt/preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%2345678901234567890123456789012345678901234567890123456789012345678901234567890
%        1         2         3         4         5         6         7         8
%\documentclass[journal,twoside,web]{ieeecolor}
\usepackage{generic}
\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
%\documentclass[letterpaper, 10 pt, conference]{ieeecolor}  % Comment this line out if you need a4paper
%\documentclass[a4paper, 10pt, conference]{ieeeconf}      % Use this line for a4 paper
%\IEEEoverridecommandlockouts                              % This command is only needed if
                                                          % you want to use the \thanks command
\overrideIEEEmargins                                      % Needed to meet printer requirements.
\pdfminorversion=6 %tell pdflatex to generate PDF in version 1.6 to resolve the error in papercept that says Font Type 3 is not allowed. If this doesn't solve the problem add this:
\usepackage[T1]{fontenc}
% See the \addtolength command later in the file to balance the column lengths
% on the last page of the document
% The following packages can be found on http:\\www.ctan.org
\usepackage{graphics} % for pdf, bitmapped graphics files
\usepackage{epsfig} % for postscript graphics files
\usepackage{mathptmx} % assumes new font selection scheme installed
\usepackage{times} % assumes new font selection scheme installed

% Customized packages outside ICRA
%\usepackage[bordercolor=white,backgroundcolor=gray!30,linecolor=black,colorinlistoftodos]{todonotes}
\usepackage[noadjust]{cite}
\renewcommand{\citedash}{--}
\usepackage{filecontents}
\usepackage{amsmath}
\DeclareMathSymbol{:}{\mathord}{operators}{"3A}  %to reduce space around colons in math mode. See https://tex.stackexchange.com/questions/432778/reduce-spacing-around-colons-in-math-mode. 
\usepackage{yhmath} %note this package will generate type 3 fonts unless you have 1.6 installed
\usepackage{mathtools} % for rotation matrix e.g. \prescript{4}{0}{R} and for summation
\usepackage{amssymb} %for trianleq symbol
\usepackage{xfrac} % needed for diagonal fraction \sfrac{a}{b} command
\usepackage{sidecap}
\input{PaperFmt/preamble_algorithm.tex}
\usepackage{graphicx}
\usepackage{tabularx}
\usepackage{subcaption}
\usepackage{multirow} 
\usepackage{leftidx} %added by Jared
\usepackage{cancel} %added by Jared
\usepackage{epsfig}
\usepackage{psfrag}
\usepackage{caption}
\usepackage[super]{nth} %to type 1st,2nd,3rd,... , use the command \nth {<number>}
\usepackage[normalem]{ulem} % to strike out
\usepackage{color}
\usepackage{xcolor} %for coloring text
\usepackage{booktabs} %nice tables
\usepackage{siunitx} %e.g. \ang{45} to show 90 degree
\usepackage{booktabs} %nice tables
\usepackage{colortbl} % to color tables
\usepackage{soul} % for strikethroughs
\usepackage{textcomp} %for a nice registered trademark, e.g. MATLAB\textsuperscript{\textregistered}
\usepackage{tikz}
% or Simulink Real-Time\texttrademark
\usepackage[noadjust]{cite} %to group citations
\usepackage{xcolor}
%\usepackage{textcomp}  %%for copyright/registered trademark symbols (see http://tex.stackexchange.com/questions/1676/how-to-get-good-looking-copyright-and-registered-symbols)
\usepackage{wasysym}  % for diameter symbol e.g. \diameter
\usepackage[mathscr]{euscript}
\usepackage{hyperref}  %this package hyperrefs to figure and equation numbers. see http://www.tug.org/applications/hyperref/manual.html
\hypersetup{
  colorlinks   = true, %true=Colours links instead of ugly boxes
  urlcolor     = blue, %Colour for external hyperlinks
  linkcolor    = blue, %Colour of internal links
  citecolor   = green %Colour of citations
}
%
\newcommand{\rework}[1]{\todo[color=yellow,inline]{#1}}
\DeclareMathOperator*{\argmin}{arg\,min} %to use argmin, ex:  \argmin_{\Psi} {f(\Psi,x)}
\newcommand{\RNum}[1]{\uppercase\expandafter{\romannumeral #1\relax}} %Roman numerals
%
%============Added by Nabil =======================
\newcommand{\Jw}{\left(\mathbf{J}_2\left(\mathbf{I}-\mathbf{J}_1^{+}\mathbf{J}_1\right)\right)}
\newcommand{\realfield}[1]{\hbox{I \kern -.5em R}^{#1}}
\newcommand {\mb}[1]{\mathbf{#1}}
\newcommand {\bs}[1]{\boldsymbol{#1}}
\newcommand{\uvec}[1]{\hat{\mathbf{#1}}}
\newcommand{\uvecf}[3]{\,^{#1}\hat{\mathbf{#2}}_{#3}}  %example: $\uvecf{3}{x}{2}
\newcommand{\Rot}{\,^{0}\mathbf{R}_{t}}
\newcommand{\Rot}[2]{{^{#1}\mathbf{R}}_{#2}}  %example: \Rot{0}{1}
\newcommand{\T}{^{\mathrm{T}}}  %shortcut for transpose
\newcommand{\qdot}[1]{\dot{\mathbf{q}}_{#1}}  %defines a macro for writing time derivatives of vectors
\newcommand{\tdot}{\dot{\mathbf{t}}}  %defines a macro for writing time derivatives of vectors
\newcommand{\xdot}{\dot{\mathbf{x}}}  %defines a macro for writing time derivatives of vectors
\newcommand{\ellhat}{\hspace{0.7mm}\hat{\hspace{-0.7mm}\bs{\ell}}}
\newcommand{\nhat}{\hat{\mathrm{\mathrm{\textbf{n}}}}}
\newcommand{\ellhatdot}{\hspace{0.7mm}\dot{\hat{\hspace{-0.7mm}\bs{\ell}}}}
%------------------Declare math operator shortcuts ------------------------
\DeclareMathOperator{\atan}{atan}
\DeclareMathOperator{\AtanTwo}{Atan2}
\DeclareMathOperator{\Argmin}{Argmin}

%% -------------------------------------------------
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[circle,minimum size=7pt,draw=black,inner sep=0.5pt](char){\scriptsize #1};}}





==> PaperFmt/preamble_algorithm.tex <==
\usepackage{algorithm,algorithmicx,algpseudocode}
% \usepackage{algorithm}
% \usepackage{algpseudocode}
%\usepackage{amssymb}

\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}

\algnewcommand\algorithmicoutput{\textbf{Output:}}
\algnewcommand\Output{\item[\algorithmicoutput]} 

%\algrenewcommand{\algorithmiccomment}[1]{\hfill$\blacktriangleright$ #1} %uncomment for black triangles

%%% example:
%\begin{algorithm}
%  \caption{Influx}
%  \label{influx}
%  \begin{algorithmic}[1]
%  \Input $p \in [0,1]$, $G$
%  \Output None \Comment{a test comment}
%  \For{$i = 0 \to 2^d-1$}\Comment{another test comment}
%    \If{$n(\nu_i) = 0$}
%      \If{ $x < p$}  \Comment{$x$ is a normal distribution number in the range of $[0,1]$}
%      \State Occupy $v_i$ site with probablility $p$
%      \EndIf
%    \EndIf
%  \EndFor
%  \end{algorithmic}
%\end{algorithm}

% for algorithmic package
%\renewcommand{\algorithmicxrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicxensure}{\textbf{Output:}}

